Using Autoencoders on Differentially Private Federated Learning GANs

Machine learning has been applied to almost all fields of computer science over the past decades. The introduction of GANs allowed for new possibilities in fields of medical research and text prediction. However, these new fields work with ever more privacy-sensitive data. In order to maintain user privacy, a combination of federated learning, differential privacy and GANs can be used to work with private data without giving away a users' privacy. Recently, two implementations of such combinations have been published: DP-Fed-Avg GAN and GS-WGAN. This paper compares their performance and introduces an alternative version of DP-Fed-Avg GAN that makes use of denoising techniques to combat the loss in accuracy that generally occurs when applying differential privacy and federated learning to GANs. We also compare the novel adaptation of denoised DP-Fed-Avg GAN to the state-of-the-art implementations in this field.

==> sections/responsible_research.tex <==
\section{Responsible Research}
During our research, at some points we had to make choices that could be considered ethically questionable. The main choice that was made was to include the results of GS-WGAN without being able to verify them. We made this choice to still be able to compare our results to the state of the art, we considered the inclusion necessary because our algorithm is based on DP-Fed-Avg GAN and thus comparing exclusively to that would be putting our results in a vacuum. To make sure there is no confusion about the results of GS-WGAN we stated that these results are unverified at multiple points in the paper. \\
\newline
Continuing from this point, we noticed that reproducing experiment results was impossible for GS-WGAN as the code was not published yet. And for DP-Fed-Avg GAN we were eventually able to get the code working, but it took a lot of effort to figure out how to set it up, mostly due to dependencies on specific Python package versions, without this being stated. These experiences were quite frustrating, that is why we will have clear instructions, including those required for a proper installation of the dependencies, in the readme file of the GitHub repository that hosts the code. \\
\newline
Another thing to consider is the impact of this research on society. We believe that this research can not be used to cause harm to anyone, as it just considers how to make private machine learning algorithms more efficient. Doing so to our knowledge can not cause anyone to be harmed as their privacy is being preserved while having better functionality in end products that use these techniques.

